The Four Dimensions of Social Network Analysis: An Overview of Research Methods, Applications, and Software Tools

Social network based applications have experienced exponential growth in recent years. One of the reasons for this rise is that this application domain offers a particularly fertile place to test and develop the most advanced computational techniques to extract valuable information from the Web. The main contribution of this work is three-fold: (1) we provide an up-to-date literature review of the state of the art on social network analysis (SNA);(2) we propose a set of new metrics based on four essential features (or dimensions) in SNA; (3) finally, we provide a quantitative analysis of a set of popular SNA tools and frameworks. We have also performed a scientometric study to detect the most active research areas and application domains in this area. This work proposes the definition of four different dimensions, namely Pattern & Knowledge discovery, Information Fusion & Integration, Scalability, and Visualization, which are used to define a set of new metrics (termed degrees) in order to evaluate the different software tools and frameworks of SNA (a set of 20 SNA-software tools are analyzed and ranked following previous metrics). These dimensions, together with the defined degrees, allow evaluating and measure the maturity of social network technologies, looking for both a quantitative assessment of them, as to shed light to the challenges and future trends in this active area.

==> sections/miscelaneous.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNA Tools for big data: Herramientas sacadas de social big data
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Structure-based Social Networks Analytics: Algorithms, Techniques, Methods, Tools and Frameworks}

{\color{blue} This section provides a description of the basic methods and algorithms related to social data analytics, network analytics, community detection, text analysis, and information diffusion. The next sections show the basic algorithms and methods that are currently being used to analyse and process information from social-based sources in previous areas.}

{\color{blue} 

\subsection{Network Analytics}

%\section{Knowledge Extraction}

%\subsection{Social Network Analysis}
%This section describes the information, or knowledge, that can be discovered or extracted from a Social Network (SN). Firstly, we characterize the different SN depending on its representation. ...
%\subsubsection{Static}
%\subsubsection{Dynamic}


{\color{blue} Today, society lives in a connected world in which communication networks are intertwined with daily life. For example, social networks are one of the most important sources of social big data; specifically, Twitter generates over 400 million tweets every day. In social networks, individuals interact with one another and provide information on their preferences and relationships, and these networks have become important tools for collective intelligence extraction. These connected networks can be represented using graphs, and network analytic methods \cite{ott2001introduction} can be applied to these graphs of networks to extract useful knowledge.

Graphs are structures formed by a set of vertices (also called nodes) and a set of edges, which are connections between pairs of vertices. The information extracted from a social network can be easily represented as a graph in which the vertices or nodes represent the users and the edges represent the relationships among them (e.g., a re-tweet of a message or a favourite mark in Twitter). a number of network metrics can be used to perform social analysis of these networks. Usually, the importance, or influence, in a social network is analysed through \textit{centrality measures}. These measures have high computational complexity in large-scale networks. Focusing on a large-scale graph analysis, a second generation of frameworks based on the MapReduce paradigm has appeared, including \textbf{Hama}, \textbf{Giraph} (based on Pregel), and \textbf{GraphLab} among others \cite{elser2013evaluation}.

%Each of these measures provide a different view about which node is important within the network \cite{zafarani2014social}: \\
%
%\begin{enumerate}
%	\item \textit{Degree Centrality}: It used to analyse the interactions between nodes identifying the \textit{most important} nodes. Those nodes with higher number of connections, or larger degree values, will be considered the most representatives. The degree centrality for a node in an undirected graph is calculated as the number of adjacent edges of this node.
%	\item \textit{Eigenvector Centrality}: Using degree centrality, nodes with more connections are considered more important. However, in real-world cases, for instance having more friends does not by itself guarantee of importance. Instead of this, having more important friends usually provides a higher importance degree. This measure tries to generalize the degree centrality based on this idea by incorporating the importance of the neighbours to detect the \textit{most influential} nodes.
%	\item \textit{Betweenness Centrality}: Other approach for measuring the centrality is to compute the number of shortest paths between a particular node and the others ones that pass through it. This measure shows how central is a node connecting any other pair of nodes into the network. Therefore it can be used to identify the nodes \textit{controlling the information flow}.
%\end{enumerate}
%
%In centrality measures, when a node is an authority (high centrality), it passes all its centrality along all of its out-links. To decrease this problem, \textit{PageRank Algorithm} divides the value of passed centrality by the number of outgoing links from that node. Thereby, each connected neighbour gets a fraction of the centrality from the source node. \\


\textbf{Pregel} \cite{Malewicz:2010:PSL:1807167.1807184} is a graph-parallel system based on the Bulk Synchronous Parallel model (BSP) \cite{Valiant:1990}. A BSP abstract computer can be interpreted as a set of processors that can follow different threads of computation in which each processor is equipped with fast local memory and interconnected by a communication network. According to this, the platform based on this model comprises three major components:
\begin{itemize}
    \item Components capable of processing and/or local memory transactions (i.e., processors).
    \item A network that routes messages between pairs of these components.
    \item A hardware facility that allows for the synchronisation of all or a subset of components.
\end{itemize}

Taking into account this model, a BSP algorithm is a sequence of global supersteps that consists of three components:

\begin{enumerate}
    \item \textit{Concurrent computation}: Every participating processor may perform local asynchronous computations.
    \item \textit{Communication}: The processes exchange data from one processor to another, facilitating remote data storage capabilities.
    \item \textit{Barrier synchronisation}: When a process reaches this point (the barrier), it waits until all other processes have reached the same barrier.
\end{enumerate}

Hama \cite{seo2010hama} and Giraph are two distributed graph processing frameworks on Hadoop that implement Pregel. The main difference between the two frameworks is the matrix computation using the MapReduce paradigm. Apache Giraph is an iterative graph processing system in which the input is a graph composed of vertices and directed edges. Computation proceeds as a sequence of iterations (supersteps). Initially, every vertex is active, and for each superstep, every active vertex invokes the ``Compute Method'' that will implement the graph algorithm that will be executed. This means that the algorithms implemented using Giraph are vertex oriented. Apache Hama does not only allow users to work with Pregel-like graph applications. This computing engine can also be used to perform compute-intensive general scientific applications and machine learning algorithms. Moreover, it currently supports YARN, which is the resource management technology that lets multiple computing frameworks run on the same Hadoop cluster using the same underlying storage. Therefore, the same data could be analysed using MapReduce or Spark.

In contrast, GraphLab is based on a different concept. Whereas Pregel is a one-vertex-centric model, this framework uses vertex-to-node mapping in which each vertex can access the state of adjacent vertices. In Pregel, the interval between two supersteps is defined by the run time of the vertex with the largest neighbourhood. Because the number of edges is usually power-law distributed, there will be few but spacious vertices in the graph. The GraphLab approach improves this splitting of vertices with large neighbourhoods across different machines and synchronises them.

Finally, Elser and Montresor \cite{elser2013evaluation} present a study of these data frameworks and their application to graph algorithms. The k-core decomposition algorithm, the goal of which is to compute the centrality of each node in a given graph, is adapted to each framework. The results obtained confirm the improvement achieved in terms of execution time for these frameworks based on Hadoop. However, from a programming paradigm point of view, the authors recommend Pregel-inspired frameworks (a vertex-centric framework), which is the better fit for graph-related problems.}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Trozo de texto sobre information fusion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Information Fusion}
The standard approach for representing SNs is the one previously described, i.e., a graph with nodes that represent the users of the networks and the edges describe the different relations between them.

Nevertheless, it is quite difficult to find a SN where the actors have only one unique type of relation. In this sense, users in a SN can interact with each other using different types of relations such as '\textit{Friendship}', '\textit{Mentions}', '\textit{Reply}'... etc.

These type of relations can be represented by a weighted graph, where the weight of each edge represent the type of relation. But this representation is not really efficient when the type of relations, the number of users and/or the number of relations growths.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bibliografía
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{bibliography}\\

Pang, B., & Lee, L. (2008). Opinion mining and sentiment analysis. Foundations and Trends® in Information Retrieval, 2(1–2), 1-135.\\
https://www.nowpublishers.com/article/Details/INR-011\\

Thelwall, M., Wilkinson, D., & Uppal, S. (2010). Data mining emotion in social network communication: Gender differences in MySpace. Journal of the American Society for Information Science and Technology, 61(1), 190-199.\\

Liang, P. W., & Dai, B. R. (2013, June). Opinion mining on social media data. In 2013 IEEE 14th International Conference on Mobile Data Management (Vol. 2, pp. 91-96). IEEE.\\

Mostafa, M. M. (2013). More than words: Social networks’ text mining for consumer brand sentiments. Expert Systems with Applications, 40(10), 4241-4251.\\

Liu, B., & Zhang, L. (2012). A survey of opinion mining and sentiment analysis. In Mining text data (pp. 415-463). Springer, Boston, MA.\\

Liu, B. (2012). Sentiment analysis and opinion mining. Synthesis lectures on human language technologies, 5(1), 1-167.\\

Liu, B., & Zhang, L. (2012). A survey of opinion mining and sentiment analysis. In Mining text data (pp. 415-463). Springer, Boston, MA.\\

Vinodhini, G., & Chandrasekaran, R. M. (2012). Sentiment analysis and opinion mining: a survey. International Journal, 2(6), 282-292.\\

Liu, B. (2015). Sentiment analysis: Mining opinions, sentiments, and emotions. Cambridge University Press.\\

Dragoni, M., Poria, S., & Cambria, E. (2018). OntoSenticNet: A commonsense ontology for sentiment analysis. IEEE Intelligent Systems, 33(3), 77-85.\\

 @inproceedings{tang2008arnetminer,
  title={Arnetminer: extraction and mining of academic social networks},
  author={Tang, Jie and Zhang, Jing and Yao, Limin and Li, Juanzi and Zhang, Li and Su, Zhong},
  booktitle={Proceedings of the 14th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={990--998},
  year={2008},
  organization={ACM}
}

@inproceedings{leskovec2008statistical,
  title={Statistical properties of community structure in large social and information networks},
  author={Leskovec, Jure and Lang, Kevin J and Dasgupta, Anirban and Mahoney, Michael W},
  booktitle={Proceedings of the 17th international conference on World Wide Web},
  pages={695--704},
  year={2008},
  organization={ACM}
}

%Freeman, L. C. (2000). Visualizing social networks. Journal of social structure, 1(1), 4.\\

Henry, N., Fekete, J. D., & McGuffin, M. J. (2007). NodeTrix: a hybrid visualization of social networks. IEEE transactions on visualization and computer graphics, 13(6), 1302-1309.\\

Handcock, M. S., Hunter, D. R., Butts, C. T., Goodreau, S. M., & Morris, M. (2008). statnet: Software tools for the representation, visualization, analysis and simulation of network data. Journal of statistical software, 24(1), 1548.\\
 
take a look at:\\
https://patents.google.com/patent/US20080104225A1/en\\

\begin{itemize}
\item \textbf{Formal definition}\\
R. Axelrod, The dissemination of culture: a model with local convergence and global polarization, J. Confl. Resolut. 41 (2) (1997) 203–226. \\

L. Solá, M. Romance, R. Criado, J. Flores, A. García del Amo, S. Boccaletti, Eigenvector centrality of nodes in multiplex networks, Chaos 23 (3) (2013)
033131.\\

Other similar networks:
\begin{itemize}
    \item Multiple networks.\\
    L. Solá, M. Romance, R. Criado, J. Flores, A. García del Amo, S. Boccaletti, Eigenvector centrality of nodes in multiplex networks, Chaos 23 (3) (2013)
033131.
    \item Temporal networks.\\
    J.P. Holme, Temporal networks, PR 519 (3) (2012) 97–125.
    \item Interconnected networks.\\
    J. Donges, H. Schultz, N. Marwan, Y. Zou, J. Kurths, Investigating the topology of interacting networks, Eur. Phys. J. B 84 (4) (2011) 635–651.
http://dx.doi.org/10.1140/epjb/e2011-10795-8.
    \item Multidimensional networks.\\
    M. Berlingerio, M. Coscia, F. Giannotti, A. Monreale, D. Pedreschi, Foundations of multidimensional network analysis, in: 2011. International
Conference on Advances in Social Networks Analysis and Mining, 2011, pp. 485–489. http://dx.doi.org/10.1109/ASONAM.2011.103.\\ 
    M. Coscia, Multidimensional network analysis (Ph.D. thesis), Universitá Degli Studi Di Pisa, Dipartimento di Informatica, 2012.
    \\ M. Berlingerio, M. Coscia, F. Giannotti, A. Monreale, D. Pedreschi, Multidimensional networks: foundations of structural analysis, World Wide Web
16 (5–6) (2013) 567–593.
    \\ M. Berlingerio, F. Pinelli, F. Calabrese, Abacus: frequent pattern mining-based community discovery in multidimensional networks, Data Min. Knowl.
Discov. 27 (3) (2013) 294–320.
    \\ M. Coscia, G. Rossetti, D. Pennacchioli, D. Ceccarelli, F. Giannotti, ‘‘you know because i know’’: a multidimensional network approach to human
resources problem, in: Proc. of the 2013 IEEE/ACM
    \item Interdependent networks.\\
    S.V. Buldyrev, R. Parshani, G. Paul, H.E. Stanley, S. Havlin, Catastrophic cascade of failures in interdependent networks, Nature 464 (7291) (2010)
1025–1028
    \\ M. Kurant, P. Thiran, Layered complex networks, Phys. Rev. Lett. 96 (2006) 138701.
    \\ R. Parshani, S.V. Buldyrev, S. Havlin, Interdependent networks: reducing the coupling strength leads to a change from a first to second order
percolation transition, Phys. Rev. Lett. 105 (4) (2010) 048701. http://dx.doi.org/10.1103/PhysRevLett.105.048701.
    \item Multilevel networks.\\
    R. Criado, J. Flores, A. García del Amo, J. Gómez-Gardeñes, M. Romance, A mathematical model for networks with structures in the mesoscale, Int. J.
Computer Math. 89 (3) (2012) 291–309.
    \item Hypernetworks. \\
    R. Criado, M. Romance, M. Vela-Pérez, Hyperstructures, a new approach to complex systems, IJBC 20 (03) (2010) 877–883.\\
    C. Berge, Hypergraphs: Combinatorics of Finite Sets, North-Holland, 1989.
    \\ D.P. Hypergraphs, in: R. Graham, M. Grötschel, L. Lovász (Eds.), Handbook of Combinatorics, North-Holland, 1995, pp. 381–432.
\\J.J., Hypernetworks for reconstructing the dynamics of multilevel systems, in: European Conference on Complex Systems, Saïd Business School,
University of Oxford, Oxford, 2006.
\\E. Estrada, J.A. Rodríguez-Velázquez, Subgraph centrality and clustering in complex hyper-networks, Physica A 364 (2006) 581–594.
\\ E.V. Konstantinova, V.A. Skorobogatov, Application of hypergraph theory in chemistry, Discrete Math. 235 (2001) 365–383.
\\ M. Karonski, T. Luczak, Random hypergraphs, in: D. Miklós, V.T. Sós, T. Szõnyi (Eds.), in: Combinatorics, Paul Erdös is Eighty, vol. 2, Bolyai Society
Mathematical Studies, Budapest, 1996, pp. 283–293.
\\ J.A. Rodríguez, On the laplacian spectrum and walk-regular hypergraphs, Linear Multilinear Algebra 51 (2003) 285–297.
\\ B. Guerra, J. Poncela, J. Gómez-Gardeñes, V. Latora, Y. Moreno, Dynamical organization towards consensus in the Axelrod model
http://dx.doi.org/10.1142/S0218127410026162.
\end{itemize}

\item \textbf{Matrices and tensor representation}\\
E. Acar, B. Yener, Unsupervised multiway data analysis: a literature survey, IEEE Trans. Knowl. Data Eng. 21 (1) (2009) 6–20.\\

M. De Domenico, A. Solé-Ribalta, E. Cozzo, M. Kivelä, Y. Moreno, M.A. Porter, S. Gómez, A. Arenas, Mathematical formulation of multilayer networks,
Phys. Rev. X 3 (2013) 041022.\\ % http://dx.doi.org/10.1103/PhysRevX.3.041022.\\

M. Kivelä, A. Arenas, M. Barthélemy, J.P. Gleeson, Y. Moreno, M.A. Porter, Multilayer networks, ArXiv e-prints. arXiv:1309.7233.\\

E. Cozzo, M. Kivelä, M. De Domenico, A. Solé, A. Arenas, S. Gómez, M.A. Porter, Y. Moreno, Clustering coefficients in multiplex networks, ArXiv e-prints.
arXiv:1307.6780.\\

APPLICATION DOMAINS:\\

T.G. Kolda, B.W. Bader, Tensor decompositions and applications, SIAM Rev. 51 (3) (2009) 455–500.\\
D.M. Dunlavy, T.G. Kolda, W.P. Kegelmeyer, Multilinear algebra for analyzing data with multiple linkages, in: J. Kepner, J. Gilbert (Eds.), Graph
Algorithms in the Language of Linear Algebra, Fundamentals of Algorithms, SIAM, Philadelphia, 2011, pp. 85–114.\\
E. Acar, D.M. Dunlavy, T.G. Kolda, Link prediction on evolving data using matrix and tensor factorizations, in: Proc. of the 2009 IEEE International
Conference on Data Mining Workshops, ICDMW ’09, IEEE Computer Society, Washington, DC, USA, 2009, pp. 262–269.\\
T.G. Kolda, J. Sun, Scalable tensor decompositions for multi-aspect data mining, in: Proc. of the 8th IEEE International Conference on Data Mining,
ICDM 2008, 2008, pp. 363–372\\

\item \textbf{Correlation in multiple networks}
\begin{itemize}
    \item Degree correlations
    \item Overlap and multidegree
    \item multistrength and inverse multiparticipation ration
    \item activities of the nodes.
\end{itemize}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Miscelaneous
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Summary and simplification of information}

Summary and simplification of information. It would increase the legibility and conciseness of the information. This would improve access to information, which is fundamental for the development of integration policies.


\subsection{User profiling}

User profiling. By analyzing the use of language, the generation of user profiles by sex, age, origin or any other discriminatory category could be automated. This capacity would be capital for the development of demographic, market and even security studies, since it would open the option to group users by their use of language.
        
 \subsection{Analysis of scientific knowledge}
        
Analysis of scientific knowledge: This knowledge can be represented as a complex system in which the different actors are the nodes of a graph, and the existing vertexes between them represent the internal relations. Thus, through the use of SNA techniques on a network of scientific knowledge, networks of authorship, intellectuals or conceptuals could be established to analyze large volumes of scientific and technical information.\\
         
 \subsection{Recommender systems}
 

